EdgeKeeper: Resilient and Lightweight Coordination for Mobile Edge Computing Systems

Mobile Edge Computing (MEC) has been gaining significant interest from first responders and tactical teams, primarily because they can employ handheld mobile devices to form a computing cluster (for computing tasks like face/scene recognition, virtual assistance) when connectivity to the cloud is not present or it is limited. High user mobility in first responder or tactical environments makes MEC challenging, as wireless links observe substantial fluctuations. Typical cloud-based coordination (e.g., ZooKeeper-based service discovery and coordination, device naming, security) needed by edge computing tasks cannot work in these environments. Driven by the need for a resilient and lightweight coordination service, in this paper, we design and implement \ek to provide cloud-like coordination for MEC systems. It provides naming, network management, application coordination, and security to distributed edge computing applications. It maintains an edge cluster among devices and intelligently stores its data on a group of replicas to guard against node failure and disconnections. We provide a full-system implementation of EdgeKeeper for Android and Linux platforms. We have integrated EdgeKeeper with existing MEC applications and performed real-world performance evaluations in a wide-area search and rescue operation conducted by first responders, which proves it to be lightweight and suitable for mobile devices.

==> applications.tex <==
\section{EdgeKeeper Applications} 

\label{sec:applications}

\subsection{RSock}
RSock runs on all devices as a Java application and takes care of the data delivery for the applications that want to use opportunistic data delivery. RSock uses GUID based device naming. \ek{} prepares a topology of the connected devices for RSock. RSock uses this topology to determine which node to select as the next hop for routing the data packets.  When sending data to a destination device, the upper layer application, such as MDFS, specifies the GUID of the destination to RSock. RScok fetches the corresponding IP from \ek{} and send the data using the IP address of the destination device. 

\subsection{MDFS: Mobile Distributed File System}
MDFS uses \ek{} for device naming and storing file metadata. MDFS uses GUID based device naming scheme. MDFS use \ek{} for service discovery and storing file metadata. All the devices running MDFS registers to the \ek{} to be found by the peers. An MDFS node fragments a file into multiple blocks and distributes across the MDFS servers to recover the file even if some of the nodes fail. The information for this file, such as the name, size, ACL, location of the blocks, etc. are archived in file metadata. The file metadata is stored in \ek{} for better reliability. 

\subsection{MStorm: Mobile Stream Processing}
MStorm uses \ek{} for device naming and cluster coordination among a group of MStorm worker nodes. A group of nodes registers themselves for MStorm service to the \ek{}. Note that, the applications communicate with the \ek{} running at the local device only. Among these nodes, one registers itself as MStorm server, and the rest of the nodes can find the GUID of the MStorm server from the service discovery API. After discovering the server GUID, the clients can look up the IP address of the server from \ek{} to communicate with the MStorm server directly. After forming MStorm group, if a device changes its IP address (e.g., switching from WiFi to LTE), the connection will be lost. At this point, a node can look up the new IP of the destination device using its GUID. 

MStorm also uses \ek{} for coordination among nodes in dynamically assigning tasks based on the workload of the participating devices. For this reason, it keeps the information about the tasks in the local \ek{}. Since MStorm communicates with the nodes within a connected edge network, it only cares about the coordination within one edge cluster. Thus, when a node leaves or a new \ek{} cluster is formed, the MStorm source node needs to reassign the tasks and put information in the \ek{}.

%\subsection{Madoop: Mobile Map Reduce}
%
%\subsection{MDFS: Mobile Distributed File System} 

==> ideas.tex <==
\section{Ideas}

{\bf Alternative approach for MDFS} A file metadata can be stored in MDFS itself i.e. each file and directory meta data can be treated as another file. The meta data for root directory would be stored in MDFS and the location of this should be known to each device.




{\bf Alternatives of Zookeeper:}

1) https://etcd.io/  use gRPC. might not be suitable for Android

2) Vert.x has long relied on Hazelcast for cluster management, and so Copycat/Atomix were originally developed for sefer cluster management in Vert.x. Vert.x clusters are not fixed to a certain size, so we needed the flexibility to be able to arbitrarily add and remove nodes without impacting the performance and availability of the cluster. So, our goal in Atomix was precisely that.

 
 We built on the Raft algorithm in Copycat/Atomix to balance the cluster membership to maintain at least n Raft voting members and replicate asynchronously to some set of non-voting members and/or heartbeat some set of stateless members. Availability is simply managed through commits to the Raft log, and the leader is responsible for replacing unavailable voting members with available non-voting members. This allows servers - including a majority of voting members - to crash without losing the availability of the cluster so long as a majority of the voting members are not lost within a short time period. Asynchronous replication - replicating from followers to asynchronous nodes - allows voting members to be replaced with non-voting members more quickly to decrease the risk of losing availability while the new member is being caught up. The process of promoting and demoting members is done in a way that ensures the number of voting members does not decrease below the desired size.
 
 3) https://github.com/atomix/atomix  -- may be very good
 
 Atomix where some subset of the nodes are active voting Raft members and a cluster manager scales the Raft portion of the cluster by replacing failed nodes with standby nodes, there's still an increased risk that the cluster can become entirely unavailable. For example, if in a cluster with three Raft nodes, two of the Raft nodes simultaneously disconnect, the cluster manager can't commit a configuration change to promote one of the standby nodes, and so the entire cluster will become unavailable until the disconnected nodes return. 
 
 -- Atomix is better partition tollerant than Hazelcast
 
 
 4) Consul - used by Harsha for Service discovery. Consul can easily be used in Android. 
 
 -- best way to manage cluster is limit the number of nodes that participate in consensus. Let's say 10 or 20. 


Thought: Data for Zookeeper is written in File. While most of the RAFT implementations keep data in memory. So, possibly when a cluster partition happens, the minority cluster loses all the data. 


==> overview.tex <==
\hl{THIS FILE NEEDS TO BE DELETED - IT'S CONTENT WAS MOVED TO design_implementation.tex}

\section{Edge Keeper Design and Implementation (4.5p)}

\label{sec:design_overview}

\subsection{Service requirements}
We aim to provide a self-sustaining computing environment at the edge such that the basic requirements are fulfilled.  Below are the main services required for an edge network 

\begin{itemize}
	\item \textbf{Dynamic Hostname mapping:} Many application, such as Madoop requires conventional host name-based DNS resolving to abstract node mobility and change in IP address. The \ek needs to abstract node mobility and dynamically translate a hostname or device ID to its corresponding IP. 
	
	\item \textbf{Service discovery and coordination:} 
	In addition to the naming service, distributed applications also require a coordination service, which provides services such as discovering service providers, synchronization, group configuration, leader election, status monitoring, critical section handling, queuing, etc.  The service discovery should provide a global view of the of available servers for a service, and when possible, provide a subset of nearby servers. 
	
	\item \textbf{Network topology discovery:} Many applications such as MStorm, RSock, MDFS require the knowledge of link qualities between peer devices to make intelligent decisions on their computation offloading or choosing nodes to store data. When these applications run link quality assessment individually, the edge network is congested by the network discovery packets. To reduce the overhead, we need a single service to discover the devices in the edge network and asses the link qualities between peer devices. 
	
	\item \textbf{Storage for application data:} Some applications such distributed file system store some metadata containing the directory structure in \ek. Conventionally, These applications store a large amount of data over multiple devices, while the file metadata (information of where file fragments are stored) is stored at a master device called name node. Since the edge network is prone to network disconnection and node failure, \ek should provide a mechanism to store the file metadata safely over a distributed group of nodes. Thus, the file metadata could be retrieved even if some of the nodes that participate in the metadata storage get disconnected.  MDFS store metadata of a file (such as file size, the locations where the file fragments are stored, etc.) in the \ek{}. A node can retrieve the file metadata from the local edge as well as the neighbor edges.
	
	\item \textbf{Authentication and Authorization:}
	User authentication is of intrinsic importance in edge networks due to its opportunistic network. The different services should only be available to the users who are already authenticated. It should try to avoid requiring any third party to authenticate a user as much as possible. Let us assume a scenario where a group of first responders is deployed in a disaster zone. Now, another responder wants to join the team. This responder's identity must be verified such that no other entity can spoof this identity. In addition, the design should ensure that the newly joined node can only access the services that are authorized for this user. 
	
\end{itemize}


%\ek{} needs to make this metadata available to the local cluster as well globally (with the best effort) for other clusters to use it.  At least,  the following operations should be permitted:
%
%\begin{itemize}
%	\item \textbf{Create a new file} After creating a file, the metadata is pushed to \ek{}. File fragments might be stored across multiple network partitions. The initial assumptions are that the \ek{}s running at separate cluster is agnostic of each other. Thus, although a file can be stored over DTN, the file metadata might not be conveyed to the remote network partition. MDFS might have to push the file metadata information to the remote cluster when a file is stored remotely. As soon as a network cluster gains connectivity with GNS, the file metadata is pushed to GNS. 
%	
%	\item \textbf{Read file}
%	This option is easy to implement. However, the complexity lies inconsistency A node from a remote cluster might have changed the content of the file. If the local cluster contains stale metadata information, the file information would not be consistent.  
%	
%	\item \textbf{Modifying a file} We consider the \ek{} to update the file metadata information lazily. Thus, if an MDFS application modifies a file and pushes the update to the \ek{}, should it indicate the modifier whether the update is committed to globally?  
%\end{itemize}



\subsection{Design Goals}
We outlined the required services by an edge network. While designing the \ek{}, we aim to achieve the following properties. 

\begin{itemize}
\item \textbf{Simple design:}
In an edge network, the mobile nodes join and leave frequently. We can not use any complex system that maintains a huge number of states and should be able to react to node joining or departure events smoothly without degrading the performance of the rest of the network. Thus, the design has to be very simple and easy to understand. 

\item \textbf{Federation:}
The design must allow several name servers to coexist independently and a user to connect to any of them. All of these servers must return the same information when connected in the same cluster or through the Internet. 

\item \textbf{Quick Response:}
The mobile nodes in edge heavily rely on naming service for updating its IP, DNS resolving, and service discovery. In the opportunistic network, data delivery is done by RSock, which makes frequent calls to map hostnames to IP addresses and vice versa. The name resolution and service discovery is a bottleneck for the upper layer applications. A name resolution should be swift if the corresponding host can find the id at the local cluster or services locally.  

\item \textbf{Scalability:}
In our design, we use replication of name records to deal with frequent node departure and association. A solution might be replicating the entire global name records to a local node. However, storing the thousands or millions of records at a node is not possible. The design should tackle the scalability issues and only store useful information that is required during the disconnection period. 
\end{itemize}

\begin{figure*}
	\centering
	\includegraphics[width=0.75\linewidth]{figures/edge_keeper_distributed.eps}
	\caption{Network components of \ek. The federated name servers manages the global view of the name records. Each organization poses control over its certification authority which issues the user certificates for registering to the \ek.}
	\label{fig:network_component}
\end{figure*}


\subsection{Design Overview}
To achieve all the goals mentioned above, we propose \ek{} a hybrid framework that deals with network disconnection swiftly while providing: a) naming; b) edge coordination, and c) security. Figure~\ref{fig:network_component} shows the main components of \ek. 


\subsubsection{Naming Service}


For persistent device naming on a global scale, it uses Global Naming Service (GNS)~\cite{sharma2014global}. GNS uses multiple name servers to deal with high name resolution rates across the globe. It replicates name records across multiple servers based on the record's lookup and update rate. \ek{} uses Auspice, an implementation of GNS for federated name record management.  It maintains Paxos for eliminating identity conflicts. The IP addresses of the GNS servers are statically assigned and known to all the mobile devices. 

The name records in \ek{} are in accordance with GNS and use the same format. Each name record is associated with a primary key: a globally unique identifier (GUID). Each name record contains an associative array of key-value pairs, as given below.

\begin{verbatim}
{   GUID: <own GUID>, 
alias: <host name for DNS>,
netaddress: [<node's IP-1> , <node's Ip-2>], 
<application-name 1>: <application-role 1>,
<application-name 2>: <application-role 2>,
last-update: <node's system time>
}
\end{verbatim}

If a device offers some service and wants it to be discovered by other nodes in the network, the service name, and the role (e.g., server, client, etc.) should be specified. Any node who wants to find a list of nodes offering a particular service will query for
\verb|getPeers(service, role)| to retrieve a list of GUIDs which contains the key-value pair as \verb|service: role|. 

\subsubsection{Replicating name record at the edge}
Unfortunately, if a GNS server gets disconnected from the federated group of GNS servers, it fails to provide services. Thus, if we use a GNS server at the edge network for name resolution, it won't serve the edge network as soon as it loses connection with the Internet. In these scenarios, we use a local cache mechanism to store the name records at the edge network. The name record updates are stored at the local cache and lazily updated to the GNS server whenever the edge network gets connected to the Internet. The cache is maintained by a group of nodes (\ek-replicas) who run consensus among themselves for consistency. In addition to maintaining the name record cache, the \ek{} also manages the authentication and authorization of a new node joining the edge network. All other nodes access the name records stored in the replicas.  


\subsubsection{Edge Coordination Service}


\subsubsection{Security}

\textbf{Authentication using Certificates:} For authentication purpose, \ek{} uses X509 certificate-based authentication \cite{housley2002internet,cooper2008internet}. Multiple third-party certification authority (CA) can be integrated with the architecture. To authenticate itself to the \ek{}, a device presents its certificate signed by a CA. The corresponding CS must be authorized by the federated server beforehand. To authorize a CA, the public certificate containing the public key of the CA must be stored in the trust store of the \ek{}. When a device presents a certificate signed by a CA and CA's public credential is found in the trust store, the device is considered authenticated by \ek{}. To obtain a signed certificate, a device first generates a private-public key pair and prepare an unsigned certificate containing the devices' credentials such as account name, organization, public key, etc. The device then requests a CA to sign this certificate. CA sign the certificate using the private key of the CA. This signed certificate can be validated by any entity possessing the public key of the corresponding CA. Alternatively, we can store the user credential such as public certificate and private key in an encrypted and password protected PKCS 12 archive \cite{nystrom2014pkcs} file (with file name extension .p12 or .pfx). This file can be distributed to the devices to, and those devices containing both the p12 file and corresponding password can authenticate itself to the \ek{}.



\subsubsection{GNS based identity record}



\subsubsection{Support of mobility}
In our project \hl{In Our Project???? - is this writeup a project report????}, the nodes observe frequent disconnection. At every re-connection, the nodes obtain new IP addresses. The \ek{} running at every node triggers updates whenever there is any change in IP address. The updated IP is stored at the federated GNS if the node can reach GNS, as well as the local \ek{} cluster. A node  X can fetch the IP of another node Y by queering \verb|getIPbyGUID(GUID_Y)| from any of the federated GNS servers. Now, if Y is not connected to the federated GNS servers, the update will only be stored in the local cluster. If X is connected to the same cluster, it can fetch the record from the \ek{} the same way it queries the federated GNS servers. 






==> soa.tex <==
%\section{Related Work}
%
%Prior work~\cite{George2012DistressNet}
